CoInDiVinE: Parallel Distributed Model Checker for Component-Based Systems

CoInDiVinE is a tool for parallel distributed model checking of interactions among components in hierarchical component-based systems. The tool extends the DiVinE framework with a new input language (component-interaction automata) and a property specification logic (CI-LTL). As the language differs from the input language of DiVinE, our tool employs a new state space generation algorithm that also supports partial order reduction. Experiments indicate that the tool has good scaling properties when run in parallel setting.

==> eptcsdata.tex <==
\providecommand{\firstpage}{63}
\providecommand{\publicationstatus}{Jiri Barnat and Keijo Heljanko (Eds.)\\ 10th International Workshop on\\ Parallel and Distributed Methods in verifiCation (PDMC 2011)\\
EPTCS 72, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.72.7}{10.4204/EPTCS.72.7}}

